Improving Diffusion Language Model Decoding through Joint Search in Generation Order and Token Space

Diffusion Language Models (DLMs) offer order-agnostic generation that can explore many possible decoding trajectories. However, current decoding methods commit to a single trajectory, limiting exploration in trajectory space. We introduce Order-Token Search to explore this space through jointly searching over generation order and token values. Its core is a likelihood estimator that scores denoising actions, enabling stable pruning and efficient exploration of diverse trajectories. Across mathematical reasoning and coding benchmarks, Order-Token Search consistently outperforms baselines on GSM8K, MATH500, Countdown, and HumanEval (3.1%, 3.8%, 7.9%, and 6.8% absolute over backbone), matching or surpassing diffu-GRPO post-trained d1-LLaDA. Our work establishes joint search as a key component for advancing decoding in DLMs.

==> 08_ref.tex <==
\section*{Ethics Statement}
This work adheres to the ICLR Code of Ethics. All experiments are conducted using publicly available benchmark datasets (GSM8K, MATH500, Countdown, and Sudoku) and pretrained models (LLaDA-8B-Instruct, LLaDA-1.5), with our contributions centered on methodological and algorithmic advancements, in particular the development of the \textbf{Order-Token Search} method which explores the joint space of generation order and token selection. The study does not involve human subjects, personal data, or other sensitive information, and no applications with a high likelihood of causing harm are considered. We have carefully examined potential risks and broader societal impacts of this research and did not identify significant ethical concerns.

\section*{Reproducibility}
We have taken deliberate steps to ensure that our work can be reliably reproduced. Detailed descriptions of the datasets and model employed are provided in Section \ref{subsec:exp-setup}, while Appendix \ref{app:settings} outlines the inference setups and hyperparameter configurations. The details of \textbf{Order-Token Search} are documented in Appendix \ref{app:algo}. Upon acceptance, we will make our algorithm implementation publicly available to support reproducibility and enable subsequent research.


{
\bibliographystyle{iclr2026_conference}
\bibliography{ref}
}

